Observational Signatures of Dust Traffic Jams in Polar-Aligning Circumbinary Disks

Misaligned circumbinary disks will produce dust traffic jams during alignment or anti-alignment to the binary orbital plane. We conduct a hydrodynamical simulation of an initially misaligned circumbinary disk undergoing polar alignment with multiple dust species. Due to differential precession between the gas and dust components, multiple dust traffic jams are produced within the disk during polar alignment. The radial locations of the dust traffic jams depend on the Stokes number of the grains, which depends on grain size. We compute the dust temperature structure using post-processing radiative transfer to produce continuum images at cm-wavelengths. Multiple distinct rings emerge in the continuum images, corresponding to the dust traffic jams. The angular resolution of upcoming observations from SKA and ngVLA will be sufficient to detect centimeter-sized grains in protoplanetary disks and resolve the widths of dust traffic jams. Therefore, dust traffic jams resulting from the differential precession of gas and dust in misaligned circumbinary disks will be a prime target for more extended wavelength observations.

==> RESPONSE.tex <==
RESPONSE: We sincerely thank the referee for the valuable suggestions that have improved the quality of our manuscript. We have incorporated the recommended revisions and detailed our responses below. We hope the revised manuscript meets the standards for publication. 



This manuscript investigates the observational signatures of dust pile-ups in polar-aligned protoplanetary disks. A number of previous studies have shown that when circumbinary disks are driven into polar alignment, differential precession between the gas and dust causes the dust to pile-up and acquire spiral arms (e.g., Aly & Lodato 2020; Longarini+ 2021; Aly+ 2021). This work shows how polar-alignment could lead to the development of substructure in protoplanetary and debris disks, such as 99 Herculis and HD 98800B, visible using the upcoming radio interferometers ngVLA and SKA. The study is interesting and timely, and it is the referee's opinion that this work could be published in ApJ Letters. However, the referee would like to see a few inclusions to help with the clarity of the authors' arguments, before the paper is accepted.

1. The angular resolution limitations should be emphasized more. Although the angular resolution of the ngVLA and SKA are deliberated in the discussion section, the referee would like to see additions to existing plots, or new plots, comparing the width of the dust rings and spiral arms generated by polar alignment, to the angular resolution. Could the beam size of ngVLA and/or SKA be displayed next to the features of Figures 3 and 4? Angular resolution limitations should also be mentioned in the Abstract and Conclusions sections.

RESPONSE: We have provided a more detailed explanation of the angular resolutions of ALMA, ngVLA, and SKA in the discussion. Additionally, we have included the impact of these angular resolutions in the abstract and conclusion. An extra panel has been added to Fig. 4, comparing the width of the dust traffic jam to the beam sizes of ALMA, ngVLA, and SKA. While the angular resolution of ALMA is too low to resolve the dust traffic jam's width, the angular resolutions of ngVLA and SKA are sufficient. The beam sizes of the telescopes are now also displayed in Fig. 3.


2. I found Figure 5 very puzzling. I believe the authors argue ngVLA and SKA are poised to detect rings and spirals from polar alignment, since St>1 grains will be able to be detected by these arrays. The referee is perplexed why St=1 grain sizes for disk toy models are being compared with the ring locations of the author's hydrodynamical simulations. Moreover, as pointed out by the authors, the ring locations depend on the grain size, so the ring locations should not be drawn as vertical lines. The referee suggests a new figure with the same marked bands, but with lines showing the locations and radial widths of rings for each grain size, along with the beam sizes of ALMA, ngVLA, and SKA.

RESPONSE:  The main reason we choose St=1 particles as the 'observable grains' in our toy model is that we expect dust rings to form when dust is sufficiently decoupled from the gas, specifically for St ≥ 1. Thus, although our hydrodynamical simulations model dust grains with St ≥ 15, in our toy model, we assume that St ≈ 1 represents a lower limit for dust ring formation. Therefore, it makes sense to compare this with the observational windows of the telescopes. We have added a sentence above equation 9 to further explain this point. Regarding the ring locations (previously shown as vertical lines in Fig. 5), we have removed them and instead highlighted the region in the disc where we expect to observe the rings based on our simulation results.


3. How substructures created by polar alignment, compared with e.g. planet, vortex generated substructures, should be briefly discussed. 

RESPONSE: We have added a paragraph in the discussion detailing substructures produced by other phenomena. 

4. The referee believes the locations of dust traffic jams plotted with vertical lines in Figures 4 and 5 should be marked in Figure 1, as it is not clear which features are being referenced.

RESPONSE:The figure would be too cluttered if we marked the locations of the dust traffic jams on Fig. 1. Instead, we have marked their final locations on Fig. 2, which correspond to the vertical lines used in Fig. 4.


5. A plot of the inclination versus time of the author's simulation should be provided, so the reader has some idea how much the disk has relaxed into polar alignment.

RESPONSE: We have updated Fig. 2 by adding an upper panel that shows the density-weighted disc tilt for both the gas and dust components. Additionally, we have included a description of the tilt evolution in Section 3.

6. The physics of the secondary traffic jams should be discussed. The referee understands the primary jams occur where the gas and dust precession rates meet, but is confused why secondary traffic jams develop. Generally, a review of the physics behind dust traffic jams would be helpful.

RESPONSE: We added a paragraph at the beginning of Section 3, detailing the physics behind the formation of the dust traffic jam. The secondary dust traffic jam forms in the same way as the primary one. As long as the gas and dust components are misaligned, the mechanism driving the formation of these traffic jams remains active.

7. The authors mention dust spirals are not present in the 6 mm image (Fig. 3), is this why dust spirals are not detected in HD 98800B? Or is ALMA's beam size a larger factor? The referee believes this should be discussed somewhere.

RESPONSE: We added a paragraph at the end of Section 5, discussing the possibilities of the non-detection of dust spirals from previous observations of the polar disc around HD 98800.

8. Stating the average stokes numbers of the simulation is not super quantitative, why not just pick a disk radial location, and state what the stokes numbers are there?

RESPONSE: We now have stated a range of the Stokes number for each dust size from rin to rout. 

9. Figure 1, but also Figure 2 and 3, appear a little bit blurry. The authors might want to increase the resolution of the png image used to create these visualizations.

RESPONSE: We have enhanced the resolution of the figures to the best of our ability.
